AfriMTE and AfriCOMET: Enhancing COMET to Embrace Under-resourced African Languages

Despite the recent progress on scaling multilingual machine translation (MT) to several under-resourced African languages, accurately measuring this progress remains challenging, since evaluation is often performed on n-gram matching metrics such as BLEU, which typically show a weaker correlation with human judgments. Learned metrics such as COMET have higher correlation; however, the lack of evaluation data with human ratings for under-resourced languages, complexity of annotation guidelines like Multidimensional Quality Metrics (MQM), and limited language coverage of multilingual encoders have hampered their applicability to African languages. In this paper, we address these challenges by creating high-quality human evaluation data with simplified MQM guidelines for error detection and direct assessment (DA) scoring for 13 typologically diverse African languages. Furthermore, we develop AfriCOMET: COMET evaluation metrics for African languages by leveraging DA data from well-resourced languages and an African-centric multilingual encoder (AfroXLM-R) to create the state-of-the-art MT evaluation metrics for African languages with respect to Spearman-rank correlation with human judgments (0.441).

==> related_work.tex <==

\section{Related Work}
@Jiayi

==> results.tex <==
% \section{Results}
% @Jiayi, Ricardo, and Sweta

% \subsection{Main Findings}

% \paragraph{Reference-based Evaluation} 
% \begin{enumerate}
%     \item \textbf{Choice of pre-trained encoders matter} As can be seen in Table~\ref{tab:spearman_main_result}: AfroXLM-R-L, a pre-trained model specifically designed for African languages, achieves the highest Spearman-rank correlation among various pre-trained models considered on a considerable portion of language pairs. Out of the 17 language pairs evaluated, AfroXLM-R-L outperforms other models by obtaining the highest correlation on 10 of these language pairs. This underlines the significance of tailored, language-specific pre-trained models in improving downstream NLP performance, especially in linguistically diverse contexts such as those found in African languages. \sa{Add afribert discussion}
%     \item \textbf{Impact of training dataset} Table~\ref{tab:afr_xlmr_result} shows the impact of using different training dataset configurations for modeling COMET. Interestingly, using ``WMT previous'' results in a higher correlation compared to using ``WMT African''. \sa{Need to add a hypothesis of why this happens: dataset size? different instructions? language pairs? translation model quality?}  Combining the two datasets for training improves Pearson correlation but hurts ranking-based correlation scores. \sa{again needs a why? needs a supporting analysis as well}
% \end{enumerate}

% % Condensed Table
% % \input{tables/main_results}

% % All results
% \input{tables/spearman_main}
% \input{tables/afr_xlmr_result}

% \paragraph{Reference-free Evaluation}
% \input{tables/ref_free_result}



% \subsection{Domain Findings}
% % yoruba domain specific analysis here





==> tables/afr_xlmr_rank.tex <==
\begin{table*}[!t]
\begin{center}
\centering
\resizebox{2.0\columnwidth}{!}{%
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
& \multicolumn{9}{c}{Training Data Settings} \\
\cmidrule{2-10}
& \multicolumn{3}{c|}{Pearson} & \multicolumn{3}{c|}{Spearman} & \multicolumn{3}{c}{Kendall}  \\
\midrule
LP & WMT African & WMT Others & WMT Combined  & WMT African & WMT Others & WMT Combined  & WMT African & WMT Others & WMT Combined \\
\midrule
ary-fra	&	3	&	1	&	1	&	2	&	1	&	1	&	2	&	1	&	1	\\
eng-arz	&	3	&	1	&	1	&	3	&	1	&	2	&	3	&	1	&	2	\\
eng-fra	&	2	&	1	&	1	&	2	&	1	&	1	&	2	&	1	&	1	\\
eng-hau	&	2	&	2	&	1	&	2	&	1	&	1	&	3	&	1	&	1	\\
eng-ibo	&	3	&	1	&	2	&	2	&	1	&	1	&	2	&	1	&	1	\\
eng-kik	&	1	&	2	&	1	&	2	&	1	&	1	&	2	&	1	&	1	\\
eng-luo	&	1	&	1	&	1	&	1	&	1	&	1	&	1	&	1	&	1	\\
eng-som	&	2	&	2	&	1	&	2	&	1	&	1	&	2	&	1	&	1	\\
eng-swh	&	2	&	1	&	1	&	2	&	1	&	1	&	3	&	2	&	2	\\
eng-twi	&	1	&	2	&	1	&	1	&	1	&	1	&	2	&	2	&	1	\\
eng-xho	&	1	&	2	&	1	&	2	&	1	&	1	&	2	&	1	&	1	\\
eng-yor	&	2	&	3	&	1	&	2	&	1	&	1	&	2	&	1	&	1	\\
eng-yor (it)	&	2	&	3	&	1	&	1	&	1	&	1	&	1	&	1	&	1	\\
eng-yor (movie)	&	2	&	3	&	1	&	2	&	1	&	1	&	2	&	1	&	1	\\
eng-yor (news)	&	2	&	1	&	1	&	2	&	1	&	1	&	2	&	1	&	1	\\
eng-yor (ted)	&	2	&	1	&	1	&	3	&	1	&	2	&	3	&	1	&	2	\\
yor-eng	&	2	&	1	&	1	&	2	&	1	&	1	&	2	&	1	&	1	\\
\midrule
Average	&	1.94	&	1.65	&	1.06	&	1.94	&	1	&	1.12	&	2.12	&	1.12	&	1.18	\\
\bottomrule
\end{tabular}
}
\end{center}
\caption{Detailed rankings from the Perm-Input hypothesis test~\citep{deutsch2021statistical} of Pearson, Spearman-rank, Kendall-rank correlation coefficients for models trained based on AfroXLM-Roberta-Large with varied training data settings. The averaged ranks are presented in the last row.}
\label{tab:afr_xlmr_rank}
\end{table*}


==> tables/afriberta.tex <==
\begin{table*}[!t]
\begin{center}
\centering
\resizebox{2.0\columnwidth}{!}{%
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
& \multicolumn{9}{c}{Training Data Settings} \\
\cmidrule{2-10}
& \multicolumn{3}{c|}{WMT African} & \multicolumn{3}{c|}{WMT Others} & \multicolumn{3}{c}{WMT Combined}  \\
\midrule
LP & Pearson & Spearman & Kendall & Pearson & Spearman & Kendall & Pearson & Spearman & Kendall \\
\midrule
ary-fra	&	0.255	&	0.214	&	0.154	&	0.409	&	0.387	&	0.275	&	0.385	&	0.384	&	0.275	\\
eng-arz	&	0.091$^*$	&	0.111$^*$	&	0.075$^*$	&	0.305	&	0.336	&	0.226	&	0.307	&	0.312	&	0.205	\\
eng-fra	&	0.341	&	0.292	&	0.202	&	0.430	&	0.446	&	0.315	&	0.418	&	0.429	&	0.301	\\
eng-hau	&	0.608	&	0.328	&	0.224	&	0.573	&	0.394	&	0.276	&	0.722	&	0.399	&	0.276	\\
eng-ibo	&	0.292	&	0.300	&	0.211	&	0.379	&	0.453	&	0.317	&	0.340	&	0.475	&	0.327	\\
eng-kik	&	0.559	&	0.229	&	0.155	&	0.463	&	0.298	&	0.207	&	0.477	&	0.231	&	0.160	\\
eng-luo	&	0.285	&	0.146	&	0.099	&	0.364	&	0.239	&	0.163	&	0.378	&	0.189	&	0.127	\\
eng-som	&	0.361	&	0.256	&	0.180	&	0.332	&	0.340	&	0.240	&	0.380	&	0.302	&	0.212	\\
eng-swh	&	0.522	&	0.464	&	0.323	&	0.665	&	0.603	&	0.434	&	0.660	&	0.558	&	0.394	\\
eng-twi	&	0.411	&	0.223	&	0.150	&	0.367	&	0.223	&	0.150	&	0.381	&	0.224	&	0.150	\\
eng-xho	&	0.391	&	0.104$^*$	&	0.082$^*$	&	0.370	&	0.151	&	0.119	&	0.461	&	0.122	&	0.096	\\
eng-yor &	0.564	&	0.180	&	0.122	&	0.388	&	0.270	&	0.186	&	0.615	&	0.218	&	0.148	\\
eng-yor (it)	&	0.721	&	0.430	&	0.303	&	0.595	&	0.374	&	0.257	&	0.766	&	0.300	&	0.207	\\
eng-yor (movie)	&	0.511	&	0.320	&	0.217	&	0.447	&	0.325	&	0.227	&	0.588	&	0.364	&	0.252	\\
eng-yor (news)	&	0.339	&	0.043$^*$	&	0.029$^*$	&	0.313	&	0.100	&	0.066	&	0.488	&	0.105	&	0.068	\\
eng-yor (ted)	&	0.403	&	0.159	&	0.109	&	0.357	&	0.227	&	0.154	&	0.534	&	0.166	&	0.114	\\
yor-eng	&	0.215	&	0.218	&	0.144	&	0.397	&	0.405	&	0.279	&	0.377	&	0.390	&	0.267	\\
\midrule
Avg. (Corr)	&	0.404	&	0.236	&	0.163	&	0.421	&	\textbf{0.328}	&	\textbf{0.229}	&	\textbf{0.487}	&	0.304	&	0.211	\\
\bottomrule
\end{tabular}
}
\end{center}
\caption{Correlation coefficients (Pearson, Spearman-rank, Kendall-rank) for models trained based on AfriBERTa-L with varied training data settings. Values marked with $^*$ indicate a p-value greater than 0.05. The average of correlation coefficient (Corr) are presented in the last row.}
\label{tab:afriberta}
\end{table*}


==> tables/corr_table.tex <==

\begin{table}[h]
\centering
 \setlength\tabcolsep{4pt}
% \scalebox{0.85}{
\begin{tabular}{lrr}
 \toprule
 \textbf{\textsc{Criteria}}  & \multicolumn{2}{c}{\textbf{\textsc{Correlation}}} \\
 & Raw score & Z-score \\
\midrule
Mistranslation & 0.62 & 0.48\\
Addition & 0.27 & 0.32\\
Omission & 0.19 & 0.20\\
Untranslated & 0.15 & 0.16 \\
\midrule
Total & 0.49 & 0.48\\
Raw score & - & 0.79 \\
  \bottomrule
 \end{tabular}
 % }
\caption{How does the presence of error types correlate with sentence-level translation quality? \sa{add length normalized correlations}}\label{tab:corr_features} 
\end{table}



==> tables/main_results.tex <==
\begin{table*}[t]
\centering
 \setlength\tabcolsep{2.5pt}
\scalebox{0.80}{
\begin{tabular}{lllrrr}
  \toprule
    \textbf{\textsc{Metric}} & \textbf{\textsc{Pre-trained Model}}& \textbf{\textsc{Train Data}} & \textbf{\textsc{Pearson}} & \textbf{\textsc{Spearman}} & \textbf{\textsc{Kendall-tau}} \\
    \midrule
     \textit{Lexical Metrics} \\
    BLEU & & & 0.231 &	0.237 &	0.164\\
    chrf++ & & & 0.350	& 0.277 & 	0.193\\

%     \addlinespace[0.2cm]
% \textit{Embedding-based Metrics} \\ 
%     BERTScore & XLM-Roberta-Large\\
%      &  Afri-XLM-Roberta-Large \\

       \addlinespace[0.2cm]
\textit{Learned Metrics} \\ 
    COMET-REF & \multirow{2}{*}{\textsc{XLM-Roberta-Large}} & WMT (general) & 0.446 & 	0.344 &	0.244 \\
     & & \quad + african  & 0.547	& 0.342	 & 0.242 \\
    
     & \multirow{2}{*}{\textsc{Info-XLM-Roberta-Large}} & WMT (general) & 0.428	& 0.371 & 	0.263 \\
     & &\quad + african  & 0.600 &	0.360 & 0.254\\

      & \multirow{2}{*}{\textsc{Afri-XLM-Roberta-Large}} & WMT (general) & 0.531 &	0.406 &	0.288 \\
     & & \quad + african  & 0.594	& 0.393 & 	0.279\\

       & \multirow{2}{*}{\textsc{Afri-BERTa-Large}} & WMT (general) & \\
     & & \quad + african  &\\

      \addlinespace[0.4cm]
      
    COMET-QE & \multirow{2}{*}{\textsc{XLM-Roberta-Large}} & WMT (general) & \\
     & & \quad + african & \\
    
     & \multirow{2}{*}{\textsc{Info-XLM-Roberta-Large}} & WMT (general) & 0.331 &	0.291	& 0.204	 \\
     & & \quad + african & 0.574 &	0.302 &	0.211\\

      & \multirow{2}{*}{\textsc{Afri-XLM-Roberta-Large}} & WMT (general) & \\
     & & \quad + african   &\\
       

  \bottomrule
 \end{tabular}
}
\caption{Average across all lps (add all languages in appendix?)}  \label{tab:main-results}
\end{table*}


==> tables/ref_free_rank.tex <==
\begin{table*}[!t]
\begin{center}
\centering
\resizebox{2.0\columnwidth}{!}{%
\begin{tabular}{l|l|c|cc|cc}
\toprule
& & Baseline & \multicolumn{2}{c|}{InfoXLM-L} & \multicolumn{2}{c}{AfroXLM-R-L} \\
Correlation & LP & CometKiwi & WMT Others & WMT Combined & WMT Others & WMT Combined \\
\midrule
% pearson	&	en-yor-movie	&	5	&	4	&	1	&	3	&	2	\\
% pearson	&	en-fra	&	1	&	1	&	1	&	2	&	2	\\
% pearson	&	en-yor-it	&	4	&	4	&	1	&	3	&	2	\\
% pearson	&	en-yor	&	3	&	3	&	1	&	2	&	1	\\
% pearson	&	en-kik	&	4	&	3	&	1	&	2	&	1	\\
% pearson	&	en-som	&	2	&	2	&	1	&	1	&	2	\\
% pearson	&	en-ibo	&	3	&	4	&	3	&	1	&	1	\\
% pearson	&	en-xho	&	2	&	2	&	1	&	1	&	1	\\
% pearson	&	en-swh	&	1	&	1	&	1	&	2	&	3	\\
% pearson	&	en-luo	&	2	&	1	&	1	&	1	&	1	\\
% pearson	&	yor-en	&	3	&	3	&	1	&	2	&	1	\\
% pearson	&	en-hau	&	4	&	3	&	1	&	2	&	2	\\
% pearson	&	en-yor-ted	&	2	&	2	&	1	&	1	&	1	\\
% pearson	&	ary-fra	&	2	&	1	&	1	&	2	&	3	\\
% pearson	&	en-twi	&	3	&	3	&	1	&	2	&	1	\\
% pearson	&	en-arz	&	1	&	1	&	2	&	2	&	2	\\
% pearson	&	en-yor-news	&	3	&	3	&	1	&	1	&	1	\\
% pearson	&	Average	&	2.65	&	2.41	&	1.18	&	1.76	&	1.59	\\
\multicolumn{1}{c|}{\multirow{18}{*}{Pearson}}	
        &	ary-fra	&	2	&	1	&	1	&	2	&	3	\\
        &	eng-arz	&	1	&	1	&	2	&	2	&	2	\\
        &	eng-fra	&	1	&	1	&	1	&	2	&	2	\\
        &	eng-hau	&	4	&	3	&	1	&	2	&	2	\\
        &	eng-ibo	&	3	&	4	&	3	&	1	&	1	\\
        &	eng-kik	&	4	&	3	&	1	&	2	&	1	\\
        &	eng-luo	&	2	&	1	&	1	&	1	&	1	\\
        &	eng-som	&	2	&	2	&	1	&	1	&	2	\\
        &	eng-swh	&	1	&	1	&	1	&	2	&	3	\\
        &	eng-twi	&	3	&	3	&	1	&	2	&	1	\\
        &	eng-xho	&	2	&	2	&	1	&	1	&	1	\\
        &	eng-yor	&	3	&	3	&	1	&	2	&	1	\\
        &	eng-yor (it)	&	4	&	4	&	1	&	3	&	2	\\
        &	eng-yor (movie)	&	5	&	4	&	1	&	3	&	2	\\
        &	eng-yor (news)	&	3	&	3	&	1	&	1	&	1	\\
        &	eng-yor (ted)	&	2	&	2	&	1	&	1	&	1	\\
        &	yor-eng	&	3	&	3	&	1	&	2	&	1	\\
 \midrule
	&	Average	&	2.65	&	2.41	&	1.18	&	1.76	&	1.59	\\
 \midrule
 \midrule
\multicolumn{1}{c|}{\multirow{18}{*}{Spearman}}
	&	ary-fra	&	1	&	1	&	1	&	1	&	1	\\
        &	eng-arz	&	2	&	1	&	2	&	3	&	3	\\
        &	eng-fra	&	2	&	1	&	1	&	2	&	3	\\
        &	eng-hau	&	3	&	3	&	3	&	1	&	2	\\
        &	eng-ibo	&	3	&	3	&	3	&	1	&	1	\\
        &	eng-kik	&	2	&	2	&	2	&	1	&	1	\\
        &	eng-luo	&	2	&	2	&	1	&	1	&	1	\\
        &	eng-som	&	2	&	3	&	2	&	1	&	2	\\
        &	eng-swh	&	1	&	1	&	1	&	2	&	3	\\
        &	eng-twi	&	2	&	2	&	1	&	2	&	2	\\
        &	eng-xho	&	3	&	2	&	1	&	1	&	1	\\
        &	eng-yor	&	3	&	2	&	2	&	1	&	1	\\
        &	eng-yor (it)	&	1	&	1	&	1	&	1	&	1	\\
        &	eng-yor (movie)	&	3	&	2	&	1	&	1	&	1	\\
        &	eng-yor (news)	&	2	&	1	&	2	&	1	&	1	\\
        &	eng-yor (ted)	&	1	&	1	&	2	&	1	&	1	\\
        &	yor-eng	&	3	&	2	&	1	&	2	&	1	\\
\midrule
	&	Average	&	2.12	&	1.76	&	1.59	&	1.35	&	1.53	\\
\bottomrule
\end{tabular}
}
\end{center}
\caption{Detailed rankings from the Perm-Input hypothesis test~\citep{deutsch2021statistical} of Pearson and Spearman-rank correlation coefficients for reference-free QE models trained based on AfroXLM-Roberta-Large and InfoXLM-Large with varied training data settings. The averaged ranks are presented in the last row.}
\label{tab:ref_free_rank}
\end{table*}

